ML-based Handover Prediction and AP Selection in Cognitive Wi-Fi Networks

Device mobility in dense Wi-Fi networks offers several challenges. Two well-known problems related to device mobility are handover prediction and access point selection. Due to the complex nature of the radio environment, analytical models may not characterize the wireless channel, which makes the solution of these problems very difficult. Recently, cognitive network architectures using sophisticated learning techniques are increasingly being applied to such problems. In this paper, we propose data-driven machine learning (ML) schemes to efficiently solve these problems in wireless LAN (WLAN) networks. The proposed schemes are evaluated and results are compared with traditional approaches to the aforementioned problems. The results report significant improvement in network performance by applying the proposed schemes. The proposed scheme for handover prediction outperforms traditional methods i.e. received signal strength method and traveling distance method by reducing the number of unnecessary handovers by 60% and 50% respectively. Similarly, in AP selection, the proposed scheme outperforms the strongest signal first and least loaded first algorithms by achieving higher throughput gains up to 9.2% and 8% respectively.

==> figures/framework.tex <==

\definecolor{bg}{rgb}{0.7, 0.75, 0.71}
\definecolor{module}{rgb}{1.0, 0.89, 0.77}
\begin{tikzpicture}[node distance=2.5cm, background rectangle/.style={fill=gray!10}, show background rectangle] 


% Controller
\node (cont) at (-3, 2) [label=left: \large SDN Controller] {\includegraphics[scale=0.08] {controller.png}};
% hub
\node (hub) [below of= cont, yshift=-3cm, label=left: \large Hub] {\includegraphics[scale=0.08] {hub.png}};
% AP
\node (ap1) [below of= hub, yshift=-1cm, label=left: \large Access Point]  {\includegraphics[scale=0.06] {ap1.png}};



%%%%%%%%%%%%%%%%%%%%%% Data Module %%%%%%%%%%%%%%%%%%
% Raw data
\node (raw) at (4, 6) [database] {Raw Data};
% Features
\node (feat) [process, right of=raw, xshift=1cm, yshift=1] {Features Extraction};
% Dataset
\node (train) [database, right of=feat, xshift=1cm, yshift=1cm] {Design Data};
\node (train2) [database, below of=train] {Eval Data};

% Box
\draw[thick,dashed, rounded corners=15pt] ($(raw.north west)+(-0.8, 1.5)$)  rectangle($(train2.south east)+(1.5,-0.6)$);
% Label
\node [text width=2.5cm] at ($(train) + (-3.0, 0.8)$)  {\large \textcolor{black}{Data Module}};



%%%%%%%%%%%%%%%%%%%%%% Control Module %%%%%%%%%%%%%%%%%%
\node (topo) [process, minimum width=4cm, right of = cont, xshift=4cm, yshift=-4cm] {Topology Management};
\node (intf) [process, minimum width=4cm, below of = topo, yshift = 1cm] {Channel Management};
\node (demd) [process, minimum width=4cm, below of = intf, yshift = 1cm] {QoS Management};
\node (powr) [process, minimum width=4cm, below of = demd, yshift = 1cm] {Energy Management};

% Box
\draw [thick,dashed, rounded corners=15pt] ($(topo.north west)+(-0.4, 0.9)$)  rectangle($(powr.south east)+(1,-0.6)$);
% Label
\node [text width=3cm] at ($(topo) + (1.1, 1.0)$)  {\large \textcolor{black}{Control Module}};



%%%%%%%%%%%%%%%%%%%%%% Machine Learning Module %%%%%%%%%%%%%%%%%%
\node (linr) [process, minimum height=1.0cm, minimum width=4cm, right of = topo, xshift=5cm] {Linear Regression};
\node (svm) [process, minimum height=1.0cm, minimum width=4cm, below of = linr, yshift=1.3cm] {Support Vector Machine};
\node (mlp) [process, minimum height=1.0cm, minimum width=4cm, below of = svm, yshift=1.3cm] {Multi layer Perceptron};
\node (rnn) [process, minimum height=1.0cm, minimum width=4cm, below of = mlp, yshift=1.3cm] {Recurrent Neural Network};
\node (kmean) [process, minimum height=1.0cm, minimum width=4cm, below of = rnn, yshift=1.3cm] {K-means};

% Box
\draw[thick,dashed, rounded corners=15pt] ($(linr.north west)+(-0.4, 1.0)$)  rectangle($(kmean.south east)+(0.8,-0.6)$);
% Label
\node [text width=3cm] at ($(linr) + (1.1, 1.0)$)  {\large \textcolor{black}{ML Module}};





%%%%%%%%%%%% Interfaces %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Data Module
\node (dec1) [round,  minimum size=0.5cm, left of = raw, xshift=0.9cm, yshift=0cm, fill=gray] {};
\node (dec2) [round,  minimum size=0.5cm, below of = train2, xshift=0cm, yshift=1.3cm, fill=gray] {};

% Control Module
\node (dec3) [round,  minimum size=0.5cm, above of = topo, xshift=0cm, yshift=-0.9cm, fill=gray] {};
\node (dec4) [round,  minimum size=0.5cm, right of = topo, xshift=0.5cm, yshift=-2.1cm, fill=gray] {};

% ML Module
\node (dec5) [round,  minimum size=0.5cm, above of = linr, xshift=0cm, yshift=-1.0cm, fill=gray] {};
\node (dec6) [round,  minimum size=0.5cm, left of = linr, xshift=0.1cm, yshift=-2.1cm, fill=gray] {};


 %%%%%%%%%%%% Links %%%%%%%%%%%%%%%%%%%%
\draw[thin]  (hub) -- (ap1);
\draw[thin]  (hub) -- (cont);
\draw[thin, ->]  (raw) -- (feat);
\draw[thin, ->]  (feat) -| (train);
\draw[thin, ->]  (feat) -| (train2);

%% Controller -> Data
%\draw[thick, line width=6pt, ->, color=gray]  (cont) |- (dec1);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffffffff}]
        (cont) |- (dec1);
\node () [minimum size=1.5cm, left of = raw, xshift=-1.0cm, yshift=0.6cm] {\large Network Parameters};


%% Controller -> Control Module
%\draw[thick, line width=6pt, <->, color=gray]  (cont) -| (dec3);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffff}]
        (cont) -| (dec3);
\node () [minimum size=1.5cm, above of = topo, xshift=1.5cm, yshift=1.0cm] {\large Call Function};


%% Data -> ML
%\draw[thick, line width=6pt, ->, color=gray]  (dec2) -- (dec5);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffffff}]
        (dec2) to (dec5);
\node () [minimum size=1.5cm, above of = linr, xshift=1.4cm, yshift=1.0cm] {\large Import Data};


%% Control -> ML
%\draw[thick, line width=6pt, <->, color=gray]  (dec4) -- (dec6);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ff}]
        (dec4) to (dec6);
\node () [minimum size=1.5cm, left of = rnn, xshift=-0.9cm, yshift=0.5cm] {\large Call Model};


\coordinate (point1) at (-3.9,0.7);
\coordinate (point2) at (-3.9,-2.8);
\draw[thick, dashed, line width=1pt, ->] (point2) -- (point1) node[midway,fill=row!30] {\emph{trigger}};
 
\coordinate (point3) at (-2.0,0.7);
\coordinate (point4) at (-2.0,-2.8);
\draw[thick, line width=1pt, ->] (point3) -- (point4) node[midway,fill=row!30] {\emph{response}};
 


%%%%%%%%%%%%%% Access %%%%%%%%%%%%%%%%%%
% UAVs
\node (uav1)  [below of = ap1, xshift=-4cm, yshift=0, label=left: \large UAV (Soft-AP)] {\includegraphics[scale=0.05] {uav.png}};
\node (uav2)  [below of = ap1, xshift=4cm, yshift=0, label=right: \large UAV (Soft-AP)] {\includegraphics[scale=0.05] {uav.png}};
\draw[snake=expanding waves, segment angle=10, color=gray!99] (ap1)  -- (uav1); 
\draw[snake=expanding waves, segment angle=10, color=gray!99] (ap1)  -- (uav2); 
  

% Cluster 1
\node (cluster1) [ground, below of= uav1, xshift=-1.0cm, yshift=0cm, fill=gray!40]{};
\node (u1) [below of = uav1, yshift = 1cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u2) [right of=u1, xshift=-1cm, yshift=-0.2cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u3) [left of=u1, xshift=0.3cm, yshift=0cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u4) [right of=u1, xshift=-0.6cm, yshift=-0.8cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u5) [left of=u1, xshift=0.9cm, yshift=-1cm] {\includegraphics[scale=0.06] {user3.png}};


% Cluster 2
\node (cluster2) [ground, below of= uav2, xshift=-1.0cm, yshift=0cm, fill=gray!40]{};
\node (u6) [below of = uav2, yshift = 1cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u7) [right of=u6, xshift=-1cm, yshift=-0.2cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u8) [left of=u6, xshift=0.3cm, yshift=0cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u9) [right of=u6, xshift=-0.6cm, yshift=-0.8cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u10) [left of=u6, xshift=0.9cm, yshift=-1cm] {\includegraphics[scale=0.06] {user3.png}};

\node (u11) [below of=ap1, xshift=-0.9cm, yshift=-0.1cm] {\includegraphics[scale=0.08] {user3.png}};
\node (u12) [below of=ap1, xshift=0.1cm, yshift=0.1cm] {\includegraphics[scale=0.08] {user3.png}};

% \begin{scope}[on background layer]
% \node[fill=bg,fit=(cont) (cluster1) (linr) (train)] {};
% \end{scope}


\end{tikzpicture}

==> figures/framework2.tex <==

\definecolor{bg}{rgb}{0.7, 0.75, 0.71}
\definecolor{module}{rgb}{1.0, 0.89, 0.77}
\begin{tikzpicture}[node distance=2.5cm, background rectangle/.style={fill=gray!10}, show background rectangle] 


% Controller
\node (cont) at (-3, 2) [label=left: \large SDN Controller] {\includegraphics[scale=0.08] {controller.png}};
% hub
\node (hub) [below of= cont, yshift=-3cm, label=left: \large Hub] {\includegraphics[scale=0.08] {hub.png}};
% AP
\node (ap1) [below of= hub, yshift=-1cm, label=left: \large Access Point]  {\includegraphics[scale=0.06] {ap1.png}};



%%%%%%%%%%%%%%%%%%%%%% Data Module %%%%%%%%%%%%%%%%%%
% Raw data
\node (raw) at (4, 6) [database] {Raw Data};
% Features
\node (feat) [process, right of=raw, xshift=1cm, yshift=1] {Features Extraction};
% Dataset
\node (train) [database, right of=feat, xshift=1cm, yshift=1cm] {Design Data};
\node (train2) [database, below of=train] {Eval Data};

% Box
\draw[thick,dashed, rounded corners=15pt] ($(raw.north west)+(-0.8, 1.5)$)  rectangle($(train2.south east)+(1.5,-0.6)$);
% Label
\node [text width=2.5cm] at ($(train) + (-3.0, 0.8)$)  {\large \textcolor{black}{Data Module}};



%%%%%%%%%%%%%%%%%%%%%% Control Module %%%%%%%%%%%%%%%%%%
\node (topo) [process, minimum width=4cm, right of = cont, xshift=4cm, yshift=-4cm] {Topology Management};
\node (intf) [process, minimum width=4cm, below of = topo, yshift = 1cm] {Channel Management};
\node (demd) [process, minimum width=4cm, below of = intf, yshift = 1cm] {QoS Management};
\node (powr) [process, minimum width=4cm, below of = demd, yshift = 1cm] {Energy Management};

% Box
\draw [thick,dashed, rounded corners=15pt] ($(topo.north west)+(-0.4, 0.9)$)  rectangle($(powr.south east)+(1,-0.6)$);
% Label
\node [text width=3cm] at ($(topo) + (1.1, 1.0)$)  {\large \textcolor{black}{Control Module}};



%%%%%%%%%%%%%%%%%%%%%% Machine Learning Module %%%%%%%%%%%%%%%%%%
\node (linr) [process, minimum height=1.0cm, minimum width=4cm, right of = topo, xshift=5cm] {Linear Regression};
\node (svm) [process, minimum height=1.0cm, minimum width=4cm, below of = linr, yshift=1.3cm] {Support Vector Machine};
\node (mlp) [process, minimum height=1.0cm, minimum width=4cm, below of = svm, yshift=1.3cm] {Multi layer Perceptron};
\node (rnn) [process, minimum height=1.0cm, minimum width=4cm, below of = mlp, yshift=1.3cm] {Recurrent Neural Network};
\node (kmean) [process, minimum height=1.0cm, minimum width=4cm, below of = rnn, yshift=1.3cm] {K-means};

% Box
\draw[thick,dashed, rounded corners=15pt] ($(linr.north west)+(-0.4, 1.0)$)  rectangle($(kmean.south east)+(0.8,-0.6)$);
% Label
\node [text width=3cm] at ($(linr) + (1.1, 1.0)$)  {\large \textcolor{black}{ML Module}};





%%%%%%%%%%%% Interfaces %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Data Module
\node (dec1) [round,  minimum size=0.5cm, left of = raw, xshift=0.9cm, yshift=0cm, fill=gray] {};
\node (dec2) [round,  minimum size=0.5cm, below of = train2, xshift=0cm, yshift=1.3cm, fill=gray] {};

% Control Module
\node (dec3) [round,  minimum size=0.5cm, above of = topo, xshift=0cm, yshift=-0.9cm, fill=gray] {};
\node (dec4) [round,  minimum size=0.5cm, right of = topo, xshift=0.5cm, yshift=-2.1cm, fill=gray] {};

% ML Module
\node (dec5) [round,  minimum size=0.5cm, above of = linr, xshift=0cm, yshift=-1.0cm, fill=gray] {};
\node (dec6) [round,  minimum size=0.5cm, left of = linr, xshift=0.1cm, yshift=-2.1cm, fill=gray] {};


 %%%%%%%%%%%% Links %%%%%%%%%%%%%%%%%%%%
\draw[thin]  (hub) -- (ap1);
\draw[thin]  (hub) -- (cont);
\draw[thin, ->]  (raw) -- (feat);
\draw[thin, ->]  (feat) -| (train);
\draw[thin, ->]  (feat) -| (train2);

%% Controller -> Data
%\draw[thick, line width=6pt, ->, color=gray]  (cont) |- (dec1);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffffffff}]
        (cont) |- (dec1);
\node () [minimum size=1.5cm, left of = raw, xshift=-1.0cm, yshift=0.6cm] {\large Network Parameters};


%% Controller -> Control Module
%\draw[thick, line width=6pt, <->, color=gray]  (cont) -| (dec3);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffff}]
        (cont) -| (dec3);
\node () [minimum size=1.5cm, above of = topo, xshift=1.5cm, yshift=1.0cm] {\large Call Function};


%% Data -> ML
%\draw[thick, line width=6pt, ->, color=gray]  (dec2) -- (dec5);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ffffff}]
        (dec2) to (dec5);
\node () [minimum size=1.5cm, above of = linr, xshift=1.4cm, yshift=1.0cm] {\large Import Data};


%% Control -> ML
%\draw[thick, line width=6pt, <->, color=gray]  (dec4) -- (dec6);
\draw [f/.tip = Fast Triangle, 
        line width=2ex, color=gray,
        {Triangle Cap[reversed] }-{[] Triangle Cap[] . ff}]
        (dec4) to (dec6);
\node () [minimum size=1.5cm, left of = rnn, xshift=-0.9cm, yshift=0.5cm] {\large Call Model};


\coordinate (point1) at (-3.9,0.7);
\coordinate (point2) at (-3.9,-2.8);
\draw[thick, dashed, line width=1pt, ->] (point2) -- (point1) node[midway,fill=row!30] {\emph{trigger}};
 
\coordinate (point3) at (-2.0,0.7);
\coordinate (point4) at (-2.0,-2.8);
\draw[thick, line width=1pt, ->] (point3) -- (point4) node[midway,fill=row!30] {\emph{response}};
 


%%%%%%%%%%%%%% Access %%%%%%%%%%%%%%%%%%
% UAVs
\node (uav1)  [below of = ap1, xshift=-4cm, yshift=0, label=left: \large UAV (Soft-AP)] {\includegraphics[scale=0.05] {uav.png}};
\node (uav2)  [below of = ap1, xshift=4cm, yshift=0, label=right: \large UAV (Soft-AP)] {\includegraphics[scale=0.05] {uav.png}};
\draw[snake=expanding waves, segment angle=10, color=gray!99] (ap1)  -- (uav1); 
\draw[snake=expanding waves, segment angle=10, color=gray!99] (ap1)  -- (uav2); 
  

% Cluster 1
\node (cluster1) [ground, below of= uav1, xshift=-1.0cm, yshift=0cm, fill=gray!40]{};
\node (u1) [below of = uav1, yshift = 1cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u2) [right of=u1, xshift=-1cm, yshift=-0.2cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u3) [left of=u1, xshift=0.3cm, yshift=0cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u4) [right of=u1, xshift=-0.6cm, yshift=-0.8cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u5) [left of=u1, xshift=0.9cm, yshift=-1cm] {\includegraphics[scale=0.06] {user3.png}};


% Cluster 2
\node (cluster2) [ground, below of= uav2, xshift=-1.0cm, yshift=0cm, fill=gray!40]{};
\node (u6) [below of = uav2, yshift = 1cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u7) [right of=u6, xshift=-1cm, yshift=-0.2cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u8) [left of=u6, xshift=0.3cm, yshift=0cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u9) [right of=u6, xshift=-0.6cm, yshift=-0.8cm] {\includegraphics[scale=0.06] {user3.png}};
\node (u10) [left of=u6, xshift=0.9cm, yshift=-1cm] {\includegraphics[scale=0.06] {user3.png}};

\node (u11) [below of=ap1, xshift=-0.9cm, yshift=-0.1cm] {\includegraphics[scale=0.08] {user3.png}};
\node (u12) [below of=ap1, xshift=0.1cm, yshift=0.1cm] {\includegraphics[scale=0.08] {user3.png}};

% \begin{scope}[on background layer]
% \node[fill=bg,fit=(cont) (cluster1) (linr) (train)] {};
% \end{scope}


\end{tikzpicture}

==> tables/datasets.tex <==

%\begin{tabular}{p{0.6cm} >{\raggedright}m{4cm}  >{\raggedright}m{2cm} >{\raggedright}p{6cm} p{3cm}}

\begin{tabular}{m{1cm} m{4.6cm}  m{2cm} m{5cm} m{3cm}}

%\arrayrulecolor{gray!50}\hline
\rowcolor{gray!10}
\textbf{Index}
& \textbf{Task}
& \textbf{Category}
& \textbf{Features}
& \textbf{Target Variable}
\\[1.3em]
\hline



1
& Throughput estimation
& Evaluation
& \begin{description} 
\item number of clients
\item Inter-arrival time 
\item distance 
\end{description}
& Throughput (Mbps)
\\[1em]
%\arrayrulecolor{gray!50}\hline

2
& Packet loss estimation
& Evaluation
& \begin{description} \item \item No. of clients \end{description}
& Packet Loss (\%)
\\[1em]
%\arrayrulecolor{gray!50}\hline

3
& Inter-Arrival Time estimation
& Evaluation
& \begin{description} \item \item Previous IAT values \end{description}
& Future IAT (s)
\\[1em]
%\arrayrulecolor{gray!50}\hline


4
& Wi-Fi channel selection
& Design
& \begin{description} \item \item ABC \end{description}
& Channel number
\\[1em]
%\arrayrulecolor{gray!50}\hline


5
& Access point selection
& Design
& \begin{description} \item \item SNR, \item AP Utilization, \item Number of clients, \item channel access Delay \end{description}
& AP MAC Address 
\\[1em]
%\arrayrulecolor{gray!50}\hline


6
& Handover prediction
& Design
& \begin{description} \item \item Past SNR values \end{description}
& Handover event
\\[1em]
%\arrayrulecolor{gray!50}\hline

7
& Network Clustering 
& Design
& \begin{description} \item \item SNR, \item euclidean distance \end{description} 
& Number of clusters
\\[1em]
%\arrayrulecolor{gray!50}\hline


8
& Optimal placement of P2P GO
& Design
& \begin{description} \item \item SNR, \item euclidean distance \end{description} 
& position
\\[1em]
%\arrayrulecolor{gray!50}\hline

9
& AP Load balancing
& Design
& \begin{description} \item \item Clients per AP, \item Average SNR \item AP Utilization   \end{description} 
& Optimum Number of Clients
\\[1em]
%\arrayrulecolor{gray!50}\hline

\end{tabular}
%}

==> tables/rel_work.tex <==


\begin{tabular}{|m{0.6cm} | >{\raggedright}m{2.5cm} | >{\raggedright}m{3cm}  |>{\raggedright}m{3cm} | m{7cm}|}


%\arrayrulecolor{gray!50}\hline
\rowcolor{gray!10}
\textbf{Ref}
& \textbf{Category}
& \textbf{Task}
& \textbf{Algorithm}
& \textbf{Model Details}
\\[1em]
\hline


%------------------------------
\cite{mariyam_2010}
& QoS Management
& Throughput Prediction
& SVR
& This study focused on throughput prediction in the Internet, however, it can be used in wireless networks by taking more wireless parameters into account.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{liu_2015}
& QoS Management
& Throughput Prediction
& SVR, RBF, MLP
& Several techniques are used.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{samba_2016}
& QoS Management
& Throughput Prediction
& GLM, NN, RF
& Datasets of input parameters (location, speed, SNR, RSRQ, RSRP, and RSSI) as features and QoS metrics (throughput, IP Set up time, HTTP set up time, average RTT) as output variables acquired for training and prediction.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{phit_2006}
& QoS Management
& Packet Inter-Arrival rate estimation
& EWMA, MLP
& Input feature is previous packet inter-arrival rates to predict future packet inter-arrival-rates.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{kajita_2014}
& Channel Management
& Channel Selection
& Linear regression
& Features or input parameters (i.e. normalized RSS, traffic bytes transmitted by interfering stations, inter-channel distance), are used to predict the output variables (i.e. MAC layer throughput and delay). The best channel which poses high throughput and less delay is selected by the access point.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{kajita}
& Channel Management
& Channel migration strategy
& SVR
& Input features (i.e. RSSI, channel utilization) are used to predict the best channel for the access point.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{chinchali}
& QoS Management
& Interference prediction
& Linear regression, MLP, K-means, Auto-encoders, 
& SNR values of previous packets are used as input features to predict the future samples.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{dhiman_2006}
& Energy Management
& Dynamic power management
& Freund and Schapire's on-line allocation algorithm \cite{freund_1997}
& The proposed scheme used power consumption in idle state, transmit state, and transition between the two states to select the optimum timeout policy.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------


\cite{li_2007}
& Topology Management
& Mobile Location estimation
& KNN
& Input features include the multipath parameters i.e. AOA, AOD and DOA while target variable is the position or coordinates of the mobile station for the given values of features.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------


\cite{kriara_2013}
& Channel Management
& Interference classification
& Categorical regression
& 802.11n features (i.e. MCS Index, spatial streams, modulation scheme, coding rate, data rate) are used to predict target variables (i.e. throughput, packet loss and fairness).
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------

\cite{suzuki_2016}
& Topology Management
& clustering Wi-Fi stations
& K-means, Fuzzy clustering, Gaussian mixture model
& Features set include MAC address, received number of frames, number of authentication frames, number of association frames, number of data frames, data rate to classify the link as one of the three possible classes (i.e. connection possible, lack of transmission speed, frequent disconnection).
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------


\cite{lin_2009}
& QoS Management
& Frame size optimization
& MLP
& Features set includes frame size and channel SNR values to predict the target variable (i.e. throughput).
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------


\cite{cadger_2017}
& QoS Management
& Neighbor prediction in MANETs
& SVM, Naive Bayes,KNN
& Features include previous location coordinates of the mobile nodes to predict the future position of the mobile node.
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------6


\cite{del_2016}
& QoS Management
& Traffic Classification
& KNN, DB-SCAN, LDA, Decision Trees, ANN, GA
& Features set (i.e. transmission power, transmission channel, estimated time of arrival (ETA) and distance between the transmitter and receiver) to predict the target variable (i.e. number of simultaneously receiving nodes).
\\[1em]
%\arrayrulecolor{gray!50}\hline
%------------------------------7


%\bottomrule
\end{tabular}
%}

